Efficient preconditioners for solving dynamical optimal transport via interior point methods

In this paper we address the numerical solution of the quadratic optimal transport problem in its dynamical form, the so-called Benamou-Brenier formulation. When solved using interior point methods, the main computational bottleneck is the solution of large saddle point linear systems arising from the associated Newton-Raphson scheme. The main purpose of this paper is to design efficient preconditioners to solve these linear systems via iterative methods. Among the proposed preconditioners, we introduce one based on the partial commutation of the operators that compose the dual Schur complement of these saddle point linear systems, which we refer as $\boldsymbol{B}\boldsymbol{B}$-preconditioner. A series of numerical tests show that the $\boldsymbol{B}\boldsymbol{B}$-preconditioner is the most efficient among those presented, despite a performance deterioration in the last steps of the interior point method. It is in fact the only one having a CPU-time that scales only slightly worse than linearly with respect to the number of unknowns used to discretize the problem.

==> figs/larger_tables_tex/sin_rec1_mesh6_h2_bb.tex <==

%\documentclass{standalone}
%\input{/home/fh/Dropbox/Dottorato/tex/l2otp/package}
%\input{/home/fh/Dropbox/Dottorato/tex/l2otp/commands}
%\begin{document}

\begin {tabular}{R{0.7cm }|R{0.44cm }R{0.44cm }R{0.44cm }R{0.5cm }|R{0.68cm }R{0.68cm }R{0.82cm }R{0.82cm }|R{0.62cm }R{0.62cm }R{0.62cm }R{0.62cm }}
\toprule
 
    \multicolumn {13}{c}{$\Triang^{0} (
    \Ncell=100,
    \coarse{\Ncell}=100)$ \quad \#DOF=(1.9e3, 3.9e3, 7.9e3, 1.6e4)}
    \\
    \midrule
     
    $\Ntime+1$ 
    & 16 & 32 & 64 & 128  
    & 16 & 32 & 64 & 128
    & 16 & 32 & 64 & 128 
    \\
    \midrule
    
    $\Relax$
    & \multicolumn {4}{c|}{\textbf {\AvgOuter}}
    & \multicolumn {4}{c|}{\textbf {\AvgCPU }}
    & \multicolumn {4}{c}{\textbf {\AvgInner }}
    \\
    \midrule
    1  & \cellcolor {gray!20}6 & 7 & 8 & 9 & \cellcolor {gray!20}1.3e0 & 2.0e0 & 3.9e0 & 7.9e0 & \cellcolor {gray!20}2.0 & 2.2 & 2.7 & 3.2\\ 
2e-1 & \cellcolor {gray!20}6 & 7 & 7 & 8 & \cellcolor {gray!20}1.0e0 & 1.9e0 & 3.8e0 & 7.5e0 & \cellcolor {gray!20}2.3 & 3.1 & 4.0 & 4.8\\ 
4e-2 & \cellcolor {gray!20}9 & 9 & 10 & 10 & \cellcolor {gray!20}1.1e0 & 2.1e0 & 3.9e0 & 7.7e0 & \cellcolor {gray!20}2.4 & 3.8 & 5.0 & 6.5\\ 
8e-3 & \cellcolor {gray!20}13 & 13 & 14 & 15 & \cellcolor {gray!20}1.2e0 & 2.0e0 & 3.9e0 & 8.0e0 & \cellcolor {gray!20}3.2 & 4.4 & 5.7 & 7.8\\ 
2e-3 & \cellcolor {gray!20}17 & 18 & 19 & 20 & \cellcolor {gray!20}1.2e0 & 2.1e0 & 4.2e0 & 8.4e0 & \cellcolor {gray!20}3.6 & 5.1 & 6.5 & 8.7\\ 
3e-4 & \cellcolor {gray!20}22 & 24 & 26 & 27 & \cellcolor {gray!20}1.2e0 & 2.2e0 & 4.4e0 & 9.0e0 & \cellcolor {gray!20}3.9 & 5.5 & 7.0 & 9.3\\ 
6e-5 & \cellcolor {gray!20}27 & 29 & 32 & 35 & \cellcolor {gray!20}1.2e0 & 2.2e0 & 4.6e0 & 9.8e0 & \cellcolor {gray!20}4.4 & 6.1 & 7.7 & 10.3\\ 
1e-5 & \cellcolor {gray!20}32 & 36 & 40 & 48 & \cellcolor {gray!20}1.3e0 & 2.3e0 & 5.0e0 & 1.1e1 & \cellcolor {gray!20}4.8 & 6.9 & 8.4 & 11.1\\ 
3e-6 & \cellcolor {gray!20}37 & 41 & 50 & 59 & \cellcolor {gray!20}1.3e0 & 2.4e0 & 5.4e0 & 1.2e1 & \cellcolor {gray!20}5.3 & 7.1 & 9.6 & 12.4\\ 
5e-7 & \cellcolor {gray!20}50 & 53 & 63 & 84 & \cellcolor {gray!20}1.4e0 & 2.6e0 & 6.0e0 & 1.4e1 & \cellcolor {gray!20}5.4 & 7.4 & 11.3 & 14.0\\ 
\toprule  & \cellcolor {gray!20}20 & 22 & 25 & 29 & \cellcolor {gray!20}1.2e0 & 2.2e0 & 4.4e0 & 9.3e0 & \cellcolor {gray!20}4.4 & 6.0 & 8.2 & 10.8\\ 
\bottomrule 
 \end{tabular}%\end{document}

==> figs/larger_tables_tex/sin_rec1_mesh6_h2_primal.tex <==

%\documentclass{standalone}
%\input{/home/fh/Dropbox/Dottorato/tex/l2otp/package}
%\input{/home/fh/Dropbox/Dottorato/tex/l2otp/commands}
%\begin{document}

\begin {tabular}{R{0.8cm }|R{0.45cm }R{0.45cm }R{0.45cm }R{0.52cm}|R{0.8cm}R{0.82cm}R{0.82cm}R{0.7cm}|R{0.7cm }R{0.7cm }R{0.7cm }R{0.7cm }}
\toprule
 
    \multicolumn {13}{c}{$\Triang^{0} (
    \Ncell=100,
    \coarse{\Ncell}=100)$ \quad \#DOFs=(1.9e3, 3.9e3, 7.9e3, 1.6e4)}
    \\
    \midrule
     
    $\Ntime\!+\!1$ 
    & 16 & 32 & 64 & 128
    & 16 & 32 & 64 & 128
    & 16 & 32 & 64 & 128
    \\
    \midrule
        
    $\Relax$
    & \multicolumn {4}{c|}{\textbf {\AvgOuter }}
    & \multicolumn {4}{c|}{\textbf {\AvgCPU }}    
    & \multicolumn {4}{c}{\textbf {\AvgInner }}
    %& \multicolumn {4}{c}{\textbf {\% Preprocess}}
    \\
    \midrule
    1  & \cellcolor {gray!20}4 & 4 & 5 & 5 & \cellcolor {gray!20}2.8e-1 & 1.2e-1 & 1.3e-1 & 1.7e-1 & \cellcolor {gray!20}2.1 & 2.9 & 3.1 & 3.6\\ 
2e-1 & \cellcolor {gray!20}4 & 5 & 5 & 5 & \cellcolor {gray!20}1.1e-1 & 1.1e-1 & 1.3e-1 & 2.3e-1 & \cellcolor {gray!20}3.2 & 4.7 & 5.5 & 6.4\\ 
4e-2 & \cellcolor {gray!20}7 & 8 & 8 & 10 & \cellcolor {gray!20}1.2e-1 & 1.4e-1 & 1.9e-1 & 3.9e-1 & \cellcolor {gray!20}5.6 & 6.5 & 8.3 & 9.1\\ 
8e-3 & \cellcolor {gray!20}9 & 12 & 19 & 20 & \cellcolor {gray!20}1.6e-1 & 2.1e-1 & 3.8e-1 & 8.5e-1 & \cellcolor {gray!20}8.8 & 12.3 & 10.3 & 13.1\\ 
2e-3 & \cellcolor {gray!20}7 & 8 & 10 & 14 & \cellcolor {gray!20}1.8e-1 & 3.1e-1 & 7.6e-1 & 2.2e0 & \cellcolor {gray!20}25.7 & 40.6 & 41.8 & 51.8\\ 
3e-4 & \cellcolor {gray!20}8 & 9 & 13 & 17 & \cellcolor {gray!20}2.6e-1 & 5.7e-1 & 1.5e0 & 4.8e0 & \cellcolor {gray!20}60.4 & 75.4 & 82.4 & 87.1\\ 
6e-5 & \cellcolor {gray!20}12 & 17 & 20 & 32 & \cellcolor {gray!20}4.3e-1 & 1.1e0 & 3.0e0 & 8.6e0 & \cellcolor {gray!20}83.8 & 89.4 & 91.8 & 95.2\\ 
1e-5 & \cellcolor {gray!20}24 & 36 & 47 & 83 & \cellcolor {gray!20}8.4e-1 & 2.6e0 & 7.6e0 & 2.4e1 & \cellcolor {gray!20}92.7 & 95.8 & 97.2 & 98.5\\ 
3e-6 & \cellcolor {gray!20}52 & 88 & 113 & 175 & \cellcolor {gray!20}1.8e0 & 6.6e0 & 1.9e1 & 5.5e1 & \cellcolor {gray!20}97.1 & 98.6 & 99.0 & 99.2\\ 
5e-7 & \cellcolor {gray!20}124 & 172 & 194 & 200 & \cellcolor {gray!20}4.5e0 & 1.3e1 & 3.2e1 & 6.8e1 & \cellcolor {gray!20}98.4 & 98.6 & 94.0 & 98.9\\ 
\midrule  & \cellcolor {gray!20}22.7 & 32.4 & 39.2 & 50.5 & \cellcolor {gray!20}7.9e-1 & 2.2e0 & 5.7e0 & 1.5e1 & \cellcolor {gray!20}82.9 & 87.3 & 85.5 & 89.6\\ 
\bottomrule 
 \end{tabular} %\end{document}

==> figs/larger_tables_tex/sin_rec1_mesh6_h2_simple.tex <==

%\documentclass{standalone}
%\input{/home/fh/Dropbox/Dottorato/tex/l2otp/package}
%\input{/home/fh/Dropbox/Dottorato/tex/l2otp/commands}
%\begin{document}

\begin {tabular}{R{0.6cm }|R{0.6cm }R{0.6cm }R{0.6cm }R{0.6cm}|R{0.82cm }R{0.82cm }R{0.82cm }R{0.82cm }|R{0.4cm }R{0.55cm }R{0.55cm }R{0.55cm }}
\toprule
 
    \multicolumn {13}{c}{$\Triang^{0} (
    \Ncell=100,
    \coarse{\Ncell}=100)$ \quad \#DOFs=(1.9e3, 3.9e3, 7.9e3, 1.6e4)}
    \\
    \midrule
    $\Ntime\!+\!1$&10 & 20 & 40 & 80&10 & 20 & 40 & 80&10 & 20 & 40 & 80\\\midrule
    $\Relax$
    & \multicolumn {4}{c|}{\textbf {\AvgOuter}}
    & \multicolumn {4}{c|}{\textbf {\AvgCPU }}
    & \multicolumn {4}{c}{\textbf {\AvgInner }}
    \\
    \midrule
    1  & \cellcolor {gray!20}34 & 34 & 32 & 34 & \cellcolor {gray!20}2.8e-1 & 1.7e-1 & 2.8e-1 & 4.4e-1 & \cellcolor {gray!20}1.0 & 1.6 & 2.0 & 2.3\\ 
2e-1 & \cellcolor {gray!20}24 & 24 & 24 & 25 & \cellcolor {gray!20}1.2e-1 & 1.6e-1 & 2.4e-1 & 4.5e-1 & \cellcolor {gray!20}1.5 & 2.4 & 3.2 & 3.9\\ 
4e-2 & \cellcolor {gray!20}22 & 22 & 22 & 22 & \cellcolor {gray!20}1.2e-1 & 1.6e-1 & 2.6e-1 & 4.6e-1 & \cellcolor {gray!20}2.3 & 3.2 & 4.2 & 5.3\\ 
8e-3 & \cellcolor {gray!20}20 & 20 & 20 & 20 & \cellcolor {gray!20}1.2e-1 & 1.7e-1 & 2.7e-1 & 5.2e-1 & \cellcolor {gray!20}2.9 & 4.0 & 5.2 & 6.7\\ 
2e-3 & \cellcolor {gray!20}19 & 19 & 20 & 20 & \cellcolor {gray!20}1.2e-1 & 1.7e-1 & 3.0e-1 & 5.8e-1 & \cellcolor {gray!20}3.5 & 5.2 & 6.4 & 7.9\\ 
3e-4 & \cellcolor {gray!20}18 & 18 & 19 & 19 & \cellcolor {gray!20}1.3e-1 & 1.8e-1 & 3.2e-1 & 6.8e-1 & \cellcolor {gray!20}4.1 & 6.0 & 7.3 & 9.5\\ 
6e-5 & \cellcolor {gray!20}16 & 18 & 18 & 19 & \cellcolor {gray!20}1.2e-1 & 1.8e-1 & 3.3e-1 & 7.6e-1 & \cellcolor {gray!20}4.5 & 6.4 & 7.6 & 10.6\\ 
1e-5 & \cellcolor {gray!20}16 & 18 & 19 & 20 & \cellcolor {gray!20}1.3e-1 & 1.9e-1 & 3.7e-1 & 8.7e-1 & \cellcolor {gray!20}5.1 & 7.1 & 9.1 & 11.2\\ 
3e-6 & \cellcolor {gray!20}17 & 18 & 20 & 32 & \cellcolor {gray!20}1.4e-1 & 2.1e-1 & 4.3e-1 & 1.4e0 & \cellcolor {gray!20}6.5 & 7.7 & 10.2 & 11.0\\ 
5e-7 & \cellcolor {gray!20}18 & 24 & 28 & 34 & \cellcolor {gray!20}1.5e-1 & 2.9e-1 & 7.3e-1 & 1.8e0 & \cellcolor {gray!20}8.0 & 8.7 & 11.8 & 14.7\\ 
\toprule  & \cellcolor {gray!20}21 & 22 & 23 & 25 & \cellcolor {gray!20}1.5e-1 & 1.9e-1 & 3.4e-1 & 7.6e-1 & \cellcolor {gray!20}3.3 & 4.6 & 6.1 & 7.8\\ 
\bottomrule 
 \end{tabular}%\end{document}

==> figs/larger_tables_tex/sin_rec1_mesh6_h3_bb.tex <==

%\documentclass{standalone}
%\input{/home/fh/Dropbox/Dottorato/tex/l2otp/package}
%\input{/home/fh/Dropbox/Dottorato/tex/l2otp/commands}
%\begin{document}

\begin {tabular}{R{0.7cm }|R{0.44cm }R{0.44cm }R{0.44cm }R{0.5cm }|R{0.68cm }R{0.68cm }R{0.82cm }R{0.82cm }|R{0.62cm }R{0.62cm }R{0.62cm }R{0.62cm }}
\toprule
 
    \multicolumn {13}{c}{$\Triang^{1} (
    \Ncell=400,
    \coarse{\Ncell}=400)$ \quad \#DOF=(7.6e3, 1.6e4, 3.2e4, 6.4e4)}
    \\
    \midrule
    1  & 6 & \cellcolor {gray!20}7 & 8 & 9 & 1.1e0 & \cellcolor {gray!20}2.1e0 & 4.2e0 & 8.4e0 & 2.0 & \cellcolor {gray!20}2.0 & 2.5 & 3.0\\ 
2e-1 & 6 & \cellcolor {gray!20}6 & 7 & 7 & 1.1e0 & \cellcolor {gray!20}2.0e0 & 4.2e0 & 8.4e0 & 2.2 & \cellcolor {gray!20}2.9 & 3.6 & 4.5\\ 
4e-2 & 13 & \cellcolor {gray!20}14 & 16 & 16 & 1.1e0 & \cellcolor {gray!20}2.3e0 & 4.7e0 & 9.4e0 & 2.3 & \cellcolor {gray!20}3.2 & 3.9 & 4.9\\ 
8e-3 & 34 & \cellcolor {gray!20}30 & 26 & 26 & 1.4e0 & \cellcolor {gray!20}2.8e0 & 5.2e0 & 1.1e1 & 3.4 & \cellcolor {gray!20}4.2 & 4.2 & 5.7\\ 
2e-3 & 39 & \cellcolor {gray!20}40 & 44 & 45 & 1.7e0 & \cellcolor {gray!20}3.4e0 & 7.0e0 & 1.5e1 & 4.6 & \cellcolor {gray!20}5.2 & 6.2 & 8.0\\ 
3e-4 & 64 & \cellcolor {gray!20}48 & 72 & 97 & 2.3e0 & \cellcolor {gray!20}3.7e0 & 1.1e1 & 2.8e1 & 5.5 & \cellcolor {gray!20}5.8 & 8.0 & 10.1\\ 
6e-5 & 105 & \cellcolor {gray!20}87 & 138 & 248 & 3.3e0 & \cellcolor {gray!20}5.5e0 & 1.7e1 & 6.6e1 & 6.2 & \cellcolor {gray!20}7.0 & 9.4 & 11.7\\ 
1e-5 & 138 & \cellcolor {gray!20}163 & \dag & \dag & 4.3e0 & \cellcolor {gray!20}1.0e1 & \dag & \dag & 7.1 & \cellcolor {gray!20}7.5 & \dag & \dag\\ 
3e-6 & 317 & \cellcolor {gray!20}400 & \dag & \dag & 9.1e0 & \cellcolor {gray!20}2.5e1 & \dag & \dag & 7.6 & \cellcolor {gray!20}8.3 & \dag & \dag\\ 
5e-7 & 400 & \cellcolor {gray!20}\dag & \dag & \dag & 1.2e1 & \cellcolor {gray!20}\dag & \dag & \dag & 7.9 & \cellcolor {gray!20}\dag & \dag & \dag\\ 
\toprule  & 100 & \cellcolor {gray!20}\dag & \dag & \dag & 3.4e0 & \cellcolor {gray!20}\dag & \dag & \dag & 7.0 & \cellcolor {gray!20}\dag & \dag & \dag\\ 
\bottomrule 
 \end{tabular}%\end{document}

==> figs/larger_tables_tex/sin_rec1_mesh6_h3_primal.tex <==

%\documentclass{standalone}
%\input{/home/fh/Dropbox/Dottorato/tex/l2otp/package}
%\input{/home/fh/Dropbox/Dottorato/tex/l2otp/commands}
%\begin{document}

\begin {tabular}{R{0.8cm }|R{0.45cm }R{0.45cm }R{0.45cm }R{0.52cm}|R{0.8cm}R{0.82cm}R{0.82cm}R{0.7cm}|R{0.7cm }R{0.7cm }R{0.7cm }R{0.7cm }}
\toprule
 
    \multicolumn {13}{c}{$\Triang^{1} (
    \Ncell=400,
    \coarse{\Ncell}=400)$ \quad \#DOFs=(7.6e3, 1.6e4, 3.2e4, 6.4e4)}
    \\
    \midrule
    1  & 4 & \cellcolor {gray!20}4 & 4 & 4 & 1.2e-1 & \cellcolor {gray!20}1.5e-1 & 2.4e-1 & 4.5e-1 & 2.1 & \cellcolor {gray!20}2.2 & 3.1 & 3.8\\ 
2e-1 & 4 & \cellcolor {gray!20}4 & 4 & 5 & 1.2e-1 & \cellcolor {gray!20}1.8e-1 & 3.0e-1 & 6.9e-1 & 3.1 & \cellcolor {gray!20}4.5 & 5.7 & 6.6\\ 
4e-2 & 6 & \cellcolor {gray!20}7 & 8 & 9 & 1.6e-1 & \cellcolor {gray!20}2.9e-1 & 5.1e-1 & 1.3e0 & 5.5 & \cellcolor {gray!20}7.8 & 8.7 & 9.4\\ 
8e-3 & 13 & \cellcolor {gray!20}19 & 17 & 31 & 2.5e-1 & \cellcolor {gray!20}7.1e-1 & 1.4e0 & 4.4e0 & 6.3 & \cellcolor {gray!20}7.6 & 12.1 & 10.8\\ 
2e-3 & 7 & \cellcolor {gray!20}10 & 12 & 15 & 4.5e-1 & \cellcolor {gray!20}1.0e0 & 3.0e0 & 7.4e0 & 21.5 & \cellcolor {gray!20}29.5 & 36.5 & 37.8\\ 
3e-4 & 7 & \cellcolor {gray!20}9 & 12 & 19 & 9.8e-1 & \cellcolor {gray!20}2.4e0 & 8.1e0 & 2.2e1 & 54.8 & \cellcolor {gray!20}71.8 & 78.9 & 85.4\\ 
6e-5 & 10 & \cellcolor {gray!20}14 & 23 & 33 & 2.2e0 & \cellcolor {gray!20}6.2e0 & 1.5e1 & 4.6e1 & 79.6 & \cellcolor {gray!20}87.0 & 92.4 & 95.1\\ 
1e-5 & 20 & \cellcolor {gray!20}28 & 47 & 77 & 4.7e0 & \cellcolor {gray!20}1.4e1 & 3.5e1 & 1.6e2 & 90.3 & \cellcolor {gray!20}94.5 & 97.1 & 98.4\\ 
3e-6 & 39 & \cellcolor {gray!20}58 & 89 & 149 & 1.0e1 & \cellcolor {gray!20}3.2e1 & 1.0e2 & 2.4e2 & 96.1 & \cellcolor {gray!20}97.8 & 98.7 & 98.7\\ 
5e-7 & 78 & \cellcolor {gray!20}114 & 172 & 200 & 2.1e1 & \cellcolor {gray!20}6.6e1 & 2.1e2 & 3.0e2 & 98.0 & \cellcolor {gray!20}99.2 & 99.2 & 98.8\\ 
\midrule  & 17.2 & \cellcolor {gray!20}24.2 & 35.1 & 48.8 & 3.5e0 & \cellcolor {gray!20}1.1e1 & 3.3e1 & 6.9e1 & 76.3 & \cellcolor {gray!20}81.0 & 86.9 & 87.3\\ 
\bottomrule 
 \end{tabular} %\end{document}

==> figs/larger_tables_tex/sin_rec1_mesh6_h3_simple.tex <==

%\documentclass{standalone}
%\input{/home/fh/Dropbox/Dottorato/tex/l2otp/package}
%\input{/home/fh/Dropbox/Dottorato/tex/l2otp/commands}
%\begin{document}

\begin {tabular}{R{0.6cm }|R{0.6cm }R{0.6cm }R{0.6cm }R{0.6cm}|R{0.82cm }R{0.82cm }R{0.82cm }R{0.82cm }|R{0.4cm }R{0.55cm }R{0.55cm }R{0.55cm }}
\toprule
 
    \multicolumn {13}{c}{$\Triang^{1} (
    \Ncell=400,
    \coarse{\Ncell}=400)$ \quad \#DOFs=(7.6e3, 1.6e4, 3.2e4, 6.4e4)}
    \\
    \midrule
    $\Ntime\!+\!1$&10 & 20 & 40 & 80&10 & 20 & 40 & 80&10 & 20 & 40 & 80\\\midrule1  & 80 & \cellcolor {gray!20}76 & 69 & 72 & 3.2e-1 & \cellcolor {gray!20}5.3e-1 & 1.1e0 & 2.3e0 & 1.0 & \cellcolor {gray!20}1.0 & 1.7 & 2.1\\ 
2e-1 & 44 & \cellcolor {gray!20}47 & 47 & 47 & 2.5e-1 & \cellcolor {gray!20}4.8e-1 & 1.1e0 & 2.4e0 & 1.3 & \cellcolor {gray!20}1.6 & 2.5 & 3.3\\ 
4e-2 & 40 & \cellcolor {gray!20}39 & 40 & 39 & 2.7e-1 & \cellcolor {gray!20}5.1e-1 & 1.3e0 & 2.9e0 & 1.9 & \cellcolor {gray!20}3.1 & 4.6 & 5.7\\ 
8e-3 & 34 & \cellcolor {gray!20}35 & 36 & 36 & 2.6e-1 & \cellcolor {gray!20}5.5e-1 & 1.5e0 & 3.8e0 & 2.9 & \cellcolor {gray!20}4.7 & 7.1 & 9.1\\ 
2e-3 & 35 & \cellcolor {gray!20}33 & 34 & 34 & 2.9e-1 & \cellcolor {gray!20}5.9e-1 & 1.7e0 & 4.7e0 & 3.8 & \cellcolor {gray!20}6.0 & 9.3 & 11.7\\ 
3e-4 & 34 & \cellcolor {gray!20}32 & 32 & 32 & 3.2e-1 & \cellcolor {gray!20}6.8e-1 & 1.9e0 & 5.5e0 & 4.6 & \cellcolor {gray!20}7.5 & 11.3 & 14.2\\ 
6e-5 & 32 & \cellcolor {gray!20}30 & 30 & 30 & 3.6e-1 & \cellcolor {gray!20}7.6e-1 & 2.2e0 & 6.2e0 & 4.8 & \cellcolor {gray!20}8.6 & 13.5 & 16.8\\ 
1e-5 & 30 & \cellcolor {gray!20}28 & 28 & 28 & 3.8e-1 & \cellcolor {gray!20}8.0e-1 & 2.3e0 & 6.8e0 & 5.0 & \cellcolor {gray!20}9.6 & 14.1 & 19.5\\ 
3e-6 & 28 & \cellcolor {gray!20}30 & 28 & 28 & 3.7e-1 & \cellcolor {gray!20}1.1e0 & 2.7e0 & 8.1e0 & 5.6 & \cellcolor {gray!20}10.7 & 15.7 & 21.6\\ 
5e-7 & 28 & \cellcolor {gray!20}36 & 32 & 32 & 4.1e-1 & \cellcolor {gray!20}1.8e0 & 4.0e0 & 1.1e1 & 6.3 & \cellcolor {gray!20}14.8 & 18.7 & 24.9\\ 
\toprule  & 40 & \cellcolor {gray!20}40 & 39 & 39 & 3.2e-1 & \cellcolor {gray!20}7.4e-1 & 1.9e0 & 5.1e0 & 3.0 & \cellcolor {gray!20}5.2 & 7.6 & 9.9\\ 
\bottomrule 
 \end{tabular}%\end{document}

==> figs/larger_tables_tex/sin_rec1_mesh6_h4_bb.tex <==

%\documentclass{standalone}
%\input{/home/fh/Dropbox/Dottorato/tex/l2otp/package}
%\input{/home/fh/Dropbox/Dottorato/tex/l2otp/commands}
%\begin{document}

\begin {tabular}{R{0.7cm }|R{0.44cm }R{0.44cm }R{0.44cm }R{0.5cm }|R{0.68cm }R{0.68cm }R{0.82cm }R{0.82cm }|R{0.62cm }R{0.62cm }R{0.62cm }R{0.62cm }}
\toprule
 
    \multicolumn {13}{c}{$\Triang^{2} (
    \Ncell=1600,
    \coarse{\Ncell}=1600)$ \quad \#DOF=(3.0e4, 6.2e4, 1.3e5, 2.5e5)}
    \\
    \midrule
    1  & 6 & 6 & \cellcolor {gray!20}8 & 9 & 1.3e0 & 2.6e0 & \cellcolor {gray!20}5.6e0 & 1.3e1 & 2.2 & 1.9 & \cellcolor {gray!20}2.3 & 2.8\\ 
2e-1 & 5 & 6 & \cellcolor {gray!20}7 & 7 & 1.3e0 & 2.7e0 & \cellcolor {gray!20}5.8e0 & 1.3e1 & 2.3 & 2.6 & \cellcolor {gray!20}3.5 & 4.2\\ 
4e-2 & 8 & 11 & \cellcolor {gray!20}12 & 11 & 1.4e0 & 3.1e0 & \cellcolor {gray!20}7.2e0 & 1.5e1 & 2.4 & 3.7 & \cellcolor {gray!20}4.6 & 5.4\\ 
8e-3 & 14 & 21 & \cellcolor {gray!20}28 & 30 & 1.7e0 & 4.1e0 & \cellcolor {gray!20}1.0e1 & 2.5e1 & 2.9 & 3.5 & \cellcolor {gray!20}3.9 & 4.3\\ 
2e-3 & 30 & 50 & \cellcolor {gray!20}44 & 54 & 2.9e0 & 8.6e0 & \cellcolor {gray!20}1.5e1 & 4.0e1 & 4.7 & 5.5 & \cellcolor {gray!20}4.3 & 4.9\\ 
3e-4 & 94 & 92 & \cellcolor {gray!20}66 & 84 & 8.3e0 & 1.8e1 & \cellcolor {gray!20}2.4e1 & 6.7e1 & 6.9 & 8.3 & \cellcolor {gray!20}5.4 & 6.3\\ 
6e-5 & 121 & 148 & \cellcolor {gray!20}94 & 121 & 1.2e1 & 3.4e1 & \cellcolor {gray!20}4.0e1 & 1.0e2 & 7.3 & 9.5 & \cellcolor {gray!20}6.4 & 7.8\\ 
1e-5 & 149 & 218 & \cellcolor {gray!20}130 & 177 & 1.8e1 & 5.8e1 & \cellcolor {gray!20}6.9e1 & 1.8e2 & 8.3 & 10.9 & \cellcolor {gray!20}8.2 & 9.5\\ 
3e-6 & 144 & 348 & \cellcolor {gray!20}181 & \dag & 1.9e1 & 1.1e2 & \cellcolor {gray!20}1.2e2 & \dag & 9.6 & 12.8 & \cellcolor {gray!20}11.8 & \dag\\ 
5e-7 & 209 & \dag & \cellcolor {gray!20}\dag & \dag & 3.3e1 & \dag & \cellcolor {gray!20}\dag & \dag & 11.7 & \dag & \cellcolor {gray!20}\dag & \dag\\ 
\toprule  & 64 & \dag & \cellcolor {gray!20}\dag & \dag & 8.0e0 & \dag & \cellcolor {gray!20}\dag & \dag & 8.4 & \dag & \cellcolor {gray!20}\dag & \dag\\ 
\bottomrule 
 \end{tabular}%\end{document}

==> figs/larger_tables_tex/sin_rec1_mesh6_h4_primal.tex <==

%\documentclass{standalone}
%\input{/home/fh/Dropbox/Dottorato/tex/l2otp/package}
%\input{/home/fh/Dropbox/Dottorato/tex/l2otp/commands}
%\begin{document}

\begin {tabular}{R{0.8cm }|R{0.45cm }R{0.45cm }R{0.45cm }R{0.52cm}|R{0.8cm}R{0.82cm}R{0.82cm}R{0.7cm}|R{0.7cm }R{0.7cm }R{0.7cm }R{0.7cm }}
\toprule
 
    \multicolumn {13}{c}{$\Triang^{2} (
    \Ncell=1600,
    \coarse{\Ncell}=1600)$ \quad \#DOFs=(3.0e4, 6.2e4, 1.3e5, 2.5e5)}
    \\
    \midrule
    1  & 4 & 3 & \cellcolor {gray!20}4 & 4 & 2.1e-1 & 3.4e-1 & \cellcolor {gray!20}7.8e-1 & 1.9e0 & 2.4 & 2.1 & \cellcolor {gray!20}2.2 & 3.4\\ 
2e-1 & 3 & 4 & \cellcolor {gray!20}4 & 4 & 2.4e-1 & 4.7e-1 & \cellcolor {gray!20}1.2e0 & 2.9e0 & 3.2 & 4.0 & \cellcolor {gray!20}5.6 & 6.4\\ 
4e-2 & 5 & 5 & \cellcolor {gray!20}6 & 7 & 3.5e-1 & 8.6e-1 & \cellcolor {gray!20}2.3e0 & 5.8e0 & 6.1 & 8.2 & \cellcolor {gray!20}10.0 & 11.6\\ 
8e-3 & 6 & 7 & \cellcolor {gray!20}7 & 9 & 6.7e-1 & 1.5e0 & \cellcolor {gray!20}4.3e0 & 1.1e1 & 10.0 & 12.8 & \cellcolor {gray!20}17.3 & 19.8\\ 
2e-3 & 6 & 8 & \cellcolor {gray!20}11 & 17 & 1.4e0 & 5.1e0 & \cellcolor {gray!20}1.1e1 & 2.9e1 & 21.8 & 26.9 & \cellcolor {gray!20}33.7 & 29.0\\ 
3e-4 & 7 & 10 & \cellcolor {gray!20}14 & 18 & 3.4e0 & 1.1e1 & \cellcolor {gray!20}3.0e1 & 7.9e1 & 54.8 & 61.7 & \cellcolor {gray!20}67.8 & 69.9\\ 
6e-5 & 10 & 14 & \cellcolor {gray!20}21 & 34 & 9.4e0 & 2.3e1 & \cellcolor {gray!20}9.3e1 & 2.0e2 & 78.2 & 85.2 & \cellcolor {gray!20}90.4 & 94.3\\ 
1e-5 & 18 & 28 & \cellcolor {gray!20}49 & 67 & 2.2e1 & 5.4e1 & \cellcolor {gray!20}2.1e2 & 4.2e2 & 88.8 & 93.4 & \cellcolor {gray!20}96.5 & 97.6\\ 
3e-6 & 36 & 64 & \cellcolor {gray!20}87 & 170 & 4.6e1 & 1.4e2 & \cellcolor {gray!20}3.0e2 & 1.2e3 & 94.0 & 97.4 & \cellcolor {gray!20}98.0 & 98.9\\ 
5e-7 & 88 & 150 & \cellcolor {gray!20}178 & \dag & 1.1e2 & 3.0e2 & \cellcolor {gray!20}6.4e2 & \dag & 97.9 & 98.8 & \cellcolor {gray!20}97.5 & \dag\\ 
\midrule  & 14.3 & 26.0 & \cellcolor {gray!20}33.2 & \dag & 1.4e1 & 4.7e1 & \cellcolor {gray!20}1.1e2 & \dag & 76.3 & 86.4 & \cellcolor {gray!20}87.7 & \dag\\ 
\bottomrule 
 \end{tabular} %\end{document}

==> figs/larger_tables_tex/sin_rec1_mesh6_h4_simple.tex <==

%\documentclass{standalone}
%\input{/home/fh/Dropbox/Dottorato/tex/l2otp/package}
%\input{/home/fh/Dropbox/Dottorato/tex/l2otp/commands}
%\begin{document}

\begin {tabular}{R{0.6cm }|R{0.6cm }R{0.6cm }R{0.6cm }R{0.6cm}|R{0.82cm }R{0.82cm }R{0.82cm }R{0.82cm }|R{0.4cm }R{0.55cm }R{0.55cm }R{0.55cm }}
\toprule
 
    \multicolumn {13}{c}{$\Triang^{2} (
    \Ncell=1600,
    \coarse{\Ncell}=1600)$ \quad \#DOFs=(3.0e4, 6.2e4, 1.3e5, 2.5e5)}
    \\
    \midrule
    $\Ntime\!+\!1$&10 & 20 & 40 & 80&10 & 20 & 40 & 80&10 & 20 & 40 & 80\\\midrule1  & 170 & 150 & \cellcolor {gray!20}157 & 161 & 1.8e0 & 3.4e0 & \cellcolor {gray!20}7.4e0 & 1.9e1 & 1.0 & 1.0 & \cellcolor {gray!20}1.0 & 1.8\\ 
2e-1 & 86 & 87 & \cellcolor {gray!20}89 & 92 & 1.2e0 & 2.6e0 & \cellcolor {gray!20}6.1e0 & 1.6e1 & 1.0 & 1.2 & \cellcolor {gray!20}1.7 & 2.6\\ 
4e-2 & 77 & 76 & \cellcolor {gray!20}75 & 75 & 1.3e0 & 3.0e0 & \cellcolor {gray!20}7.9e0 & 2.3e1 & 1.8 & 2.4 & \cellcolor {gray!20}4.0 & 5.9\\ 
8e-3 & 66 & 67 & \cellcolor {gray!20}66 & 66 & 1.3e0 & 3.6e0 & \cellcolor {gray!20}9.7e0 & 3.0e1 & 3.0 & 4.4 & \cellcolor {gray!20}6.7 & 10.0\\ 
2e-3 & 70 & 66 & \cellcolor {gray!20}63 & 61 & 1.8e0 & 4.5e0 & \cellcolor {gray!20}1.3e1 & 4.4e1 & 3.9 & 6.6 & \cellcolor {gray!20}11.0 & 17.5\\ 
3e-4 & 68 & 69 & \cellcolor {gray!20}66 & 63 & 2.4e0 & 5.8e0 & \cellcolor {gray!20}1.8e1 & 6.2e1 & 4.5 & 8.6 & \cellcolor {gray!20}14.4 & 24.7\\ 
6e-5 & 70 & 66 & \cellcolor {gray!20}64 & 64 & 3.2e0 & 7.4e0 & \cellcolor {gray!20}2.2e1 & 8.8e1 & 4.8 & 11.3 & \cellcolor {gray!20}18.7 & 33.7\\ 
1e-5 & 66 & 60 & \cellcolor {gray!20}61 & 58 & 2.9e0 & 9.2e0 & \cellcolor {gray!20}2.6e1 & 9.7e1 & 5.0 & 13.9 & \cellcolor {gray!20}22.8 & 38.0\\ 
3e-6 & 65 & 58 & \cellcolor {gray!20}57 & 55 & 3.0e0 & 1.2e1 & \cellcolor {gray!20}3.5e1 & 1.0e2 & 5.5 & 16.2 & \cellcolor {gray!20}27.2 & 39.0\\ 
5e-7 & 68 & 52 & \cellcolor {gray!20}52 & 60 & 3.5e0 & 1.8e1 & \cellcolor {gray!20}4.7e1 & 1.3e2 & 5.9 & 19.5 & \cellcolor {gray!20}33.8 & 39.3\\ 
\toprule  & 83 & 79 & \cellcolor {gray!20}79 & 80 & 2.1e0 & 6.4e0 & \cellcolor {gray!20}1.7e1 & 5.4e1 & 2.8 & 6.0 & \cellcolor {gray!20}9.5 & 14.4\\ 
\bottomrule 
 \end{tabular}%\end{document}

==> figs/larger_tables_tex/sin_rec1_mesh6_h5_primal.tex <==

%\documentclass{standalone}
%\input{/home/fh/Dropbox/Dottorato/tex/l2otp/package}
%\input{/home/fh/Dropbox/Dottorato/tex/l2otp/commands}
%\begin{document}

\begin {tabular}{R{0.8cm }|R{0.45cm }R{0.45cm }R{0.45cm }R{0.52cm}|R{0.8cm}R{0.82cm}R{0.82cm}R{0.7cm}|R{0.7cm }R{0.7cm }R{0.7cm }R{0.7cm }}
\toprule
 
    \multicolumn {13}{c}{$\Triang^{3} (
    \Ncell=6400,
    \coarse{\Ncell}=6400)$ \quad \#DOFs=(1.2e5, 2.5e5, 5.1e5, 1.0e6)}
    \\
    \midrule
    1  & 3 & 3 & 3 & \cellcolor {gray!20}3 & 6.2e-1 & 1.4e0 & 3.0e0 & \cellcolor {gray!20}7.5e0 & 2.7 & 2.7 & 2.1 & \cellcolor {gray!20}2.9\\ 
2e-1 & 3 & 3 & 3 & \cellcolor {gray!20}4 & 7.7e-1 & 1.8e0 & 4.4e0 & \cellcolor {gray!20}1.2e1 & 3.5 & 3.7 & 4.8 & \cellcolor {gray!20}6.6\\ 
4e-2 & 4 & 4 & 5 & \cellcolor {gray!20}6 & 1.2e0 & 3.1e0 & 9.3e0 & \cellcolor {gray!20}2.6e1 & 6.9 & 6.9 & 9.8 & \cellcolor {gray!20}12.8\\ 
8e-3 & 5 & 6 & 7 & \cellcolor {gray!20}8 & 2.4e0 & 5.3e0 & 1.6e1 & \cellcolor {gray!20}4.9e1 & 13.9 & 10.5 & 16.1 & \cellcolor {gray!20}19.9\\ 
2e-3 & 6 & 7 & 9 & \cellcolor {gray!20}12 & 1.1e1 & 1.7e1 & 4.0e1 & \cellcolor {gray!20}1.1e2 & 37.5 & 26.3 & 30.7 & \cellcolor {gray!20}34.2\\ 
3e-4 & 7 & 8 & 10 & \cellcolor {gray!20}15 & 1.9e1 & 3.9e1 & 9.0e1 & \cellcolor {gray!20}2.6e2 & 70.4 & 59.0 & 57.1 & \cellcolor {gray!20}61.9\\ 
6e-5 & 13 & 14 & 17 & \cellcolor {gray!20}26 & 3.8e1 & 8.0e1 & 2.1e2 & \cellcolor {gray!20}6.2e2 & 84.8 & 83.2 & 83.0 & \cellcolor {gray!20}84.2\\ 
1e-5 & 24 & 26 & 36 & \cellcolor {gray!20}58 & 8.4e1 & 1.8e2 & 6.5e2 & \cellcolor {gray!20}1.6e3 & 91.3 & 92.7 & 94.8 & \cellcolor {gray!20}96.6\\ 
3e-6 & 56 & 58 & 109 & \cellcolor {gray!20}162 & 2.2e2 & 4.6e2 & 2.5e3 & \cellcolor {gray!20}4.3e3 & 96.3 & 96.3 & 98.6 & \cellcolor {gray!20}98.8\\ 
5e-7 & \dag & 158 & 185 & \cellcolor {gray!20}\dag & \dag & 1.4e3 & 3.8e3 & \cellcolor {gray!20}\dag & \dag & 97.4 & 97.1 & \cellcolor {gray!20}\dag\\ 
\midrule  & \dag & 21.3 & 33.4 & \cellcolor {gray!20}\dag & \dag & 1.5e2 & 6.2e2 & \cellcolor {gray!20}\dag & \dag & 84.0 & 88.4 & \cellcolor {gray!20}\dag\\ 
\bottomrule 
 \end{tabular} %\end{document}

==> figs/larger_tables_tex/sin_rec1_mesh6_h5_simple.tex <==

%\documentclass{standalone}
%\input{/home/fh/Dropbox/Dottorato/tex/l2otp/package}
%\input{/home/fh/Dropbox/Dottorato/tex/l2otp/commands}
%\begin{document}

\begin {tabular}{R{0.6cm }|R{0.6cm }R{0.6cm }R{0.6cm }R{0.6cm}|R{0.82cm }R{0.82cm }R{0.82cm }R{0.82cm }|R{0.4cm }R{0.55cm }R{0.55cm }R{0.55cm }}
\toprule
 
    \multicolumn {13}{c}{$\Triang^{3} (
    \Ncell=6400,
    \coarse{\Ncell}=6400)$ \quad \#DOFs=(1.2e5, 2.5e5, 5.1e5, 1.0e6)}
    \\
    \midrule
    $\Ntime\!+\!1$&10 & 20 & 40 & 80&10 & 20 & 40 & 80&10 & 20 & 40 & 80\\\midrule1  & 328 & 332 & 337 & \cellcolor {gray!20}328 & 1.4e1 & 3.1e1 & 7.4e1 & \cellcolor {gray!20}1.6e2 & 1.0 & 1.0 & 1.0 & \cellcolor {gray!20}1.0\\ 
2e-1 & 159 & 160 & 173 & \cellcolor {gray!20}200 & 8.6e0 & 1.9e1 & 4.9e1 & \cellcolor {gray!20}1.5e2 & 1.0 & 1.1 & 1.1 & \cellcolor {gray!20}1.6\\ 
4e-2 & 134 & 156 & 151 & \cellcolor {gray!20}146 & 9.0e0 & 2.3e1 & 5.8e1 & \cellcolor {gray!20}1.8e2 & 1.8 & 1.9 & 2.7 & \cellcolor {gray!20}4.3\\ 
8e-3 & 116 & 118 & 123 & \cellcolor {gray!20}117 & 9.6e0 & 2.3e1 & 6.5e1 & \cellcolor {gray!20}2.1e2 & 3.0 & 3.3 & 4.8 & \cellcolor {gray!20}7.6\\ 
2e-3 & 130 & 104 & 110 & \cellcolor {gray!20}112 & 1.5e1 & 3.1e1 & 9.9e1 & \cellcolor {gray!20}3.8e2 & 5.3 & 5.6 & 9.9 & \cellcolor {gray!20}16.9\\ 
3e-4 & 120 & 108 & 106 & \cellcolor {gray!20}111 & 2.1e1 & 4.6e1 & 1.4e2 & \cellcolor {gray!20}5.9e2 & 6.9 & 8.0 & 14.9 & \cellcolor {gray!20}29.5\\ 
6e-5 & 124 & 116 & 117 & \cellcolor {gray!20}114 & 3.0e1 & 7.1e1 & 2.0e2 & \cellcolor {gray!20}6.6e2 & 7.8 & 9.5 & 20.2 & \cellcolor {gray!20}37.1\\ 
1e-5 & 137 & 120 & 122 & \cellcolor {gray!20}119 & 4.2e1 & 9.3e1 & 2.8e2 & \cellcolor {gray!20}7.2e2 & 8.4 & 10.2 & 27.6 & \cellcolor {gray!20}39.5\\ 
3e-6 & 140 & 113 & 103 & \cellcolor {gray!20}119 & 5.5e1 & 1.0e2 & 3.3e2 & \cellcolor {gray!20}7.7e2 & 9.3 & 10.9 & 35.5 & \cellcolor {gray!20}39.9\\ 
5e-7 & 141 & 106 & 93 & \cellcolor {gray!20}123 & 6.6e1 & 1.4e2 & 4.6e2 & \cellcolor {gray!20}9.2e2 & 10.1 & 12.0 & 39.4 & \cellcolor {gray!20}40.0\\ 
\toprule  & 161 & 154 & 153 & \cellcolor {gray!20}162 & 2.2e1 & 4.9e1 & 1.6e2 & \cellcolor {gray!20}4.2e2 & 3.9 & 4.2 & 9.7 & \cellcolor {gray!20}13.6\\ 
\bottomrule 
 \end{tabular}%\end{document}

==> shared.tex <==
\usepackage{cleveref}
\input{package.tex}
\input{commands.tex}
\input{style.tex}


% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
%\newsiamremark{hypothesis}{Hypothesis}
%\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}



% Sets running headers as well as PDF title and authors
\headers{}{E. Facca, G. Todeschi, A. Natale and M. Benzi}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{
  Efficient preconditioners for solving dynamical optimal transport via interior point methods
}

% Authors: full names plus addresses.
\author{
  Enrico Facca\thanks{
  Department of Mathematics,
    University of Bergen,
    Bergen, Norway
    (\email{enrico.facca@uib.no}).
  }
  \and
  Gabriele Todeschi\thanks{
    Univ. Grenoble Alpes, ISTerre, F-38058 Grenoble, France
    (\email{gabriele.todeschi@univ-grenoble-alpes.fr}).
  }
  \and
  Andrea Natale\thanks{
  	Univ. Lille, Inria, CNRS, UMR 8524 - Laboratoire Paul Painlev\'e,
  	F-59000 Lille, France
  	(\email{andrea.natale@inria.fr}).
  }
   \and
   Michele Benzi\thanks{
     Scuola Normale Superiore,
     Piazza dei Cavalieri, 7, 56126 Pisa, Italy  
     (\email{michele.benzi@sns.it}).
   }
}

\usepackage{amsopn}

